Inspect, Understand, Overcome: A Survey of Practical Methods for AI Safety

The use of deep neural networks (DNNs) in safety-critical applications like mobile health and autonomous driving is challenging due to numerous model-inherent shortcomings. These shortcomings are diverse and range from a lack of generalization over insufficient interpretability to problems with malicious inputs. Cyber-physical systems employing DNNs are therefore likely to suffer from safety concerns. In recent years, a zoo of state-of-the-art techniques aiming to address these safety concerns has emerged. This work provides a structured and broad overview of them. We first identify categories of insufficiencies to then describe research activities aiming at their detection, quantification, or mitigation. Our paper addresses both machine learning experts and safety engineers: The former ones might profit from the broad range of machine learning topics covered and discussions on limitations of recent methods. The latter ones might gain insights into the specifics of modern ML methods. We moreover hope that our contribution fuels discussions on desiderata for ML systems and strategies on how to propel existing approaches accordingly.

==> safety_metrics/safety_metrics.tex <==
Metrics are used to assess safety aspects in the context of DNNs. This
assessment provides a measurement and an interpretation of the
measurement result. Safety aspects refers to systematic and latent
weaknesses of the DNN - also called DNN insufficiencies,
which must be addressed in the context of a safety argumentation
\cite{saemann_strategy_2020,schwalbe_survey_2020,burton_confidence_2019}.
\cite{saemann_strategy_2020} provides a possible division of DNN
insufficiencies for a perception function for HAD systems and suggests
a general categorization of potential evaluation metrics. Based on the
measurement results, safety mechanisms, which are used to mitigate DNN
insufficiencies, can be evaluated and compared. The definition of an
exact threshold or range of values depends on the function in which
the DNN is embedded (\eg in an emergency breaking system),
and may take into account severity levels of considered situations
\cite{cheng_towards_2018}. 
\cite{burton_confidence_2019} provides a strategy to evaluate the
contribution of performance metric values in the assurance case of an
autonomous driving system. 
\cite{schwalbe_survey_2020} allocates metrics to categories of safety
requirements for DNNs. 
A small collection of diverse specialized metrics is suggested in
\cite{cheng_towards_2018}.
The described neuron coverage metrics can be used for an estimation of
the latent feature space coverage. 
A broader overview over such metrics
is given in \cite{odena_tensorfuzz_2019}. 
For easier addressing of the metrics in the safety argumentation we
divide the metrics into \emph{data}, \emph{performance},
\emph{robustness}, and \emph{interpretability} metrics.

The \emph{data} with which the DNN is trained and tested play a
decisive role. All metrics that measure the quality aspects of
acquired training and test data fall under the category data metrics. 
Examples of properties to measure are
distribution shift,
realism of synthetic data (\eg Peak-Signal-to-Noise Ratio),
independence of train, validation and test datasets,
outlier detection,
input space / ODD coverage, and
annotation quality (mitigation of human labeling error).
For example, the latter can be measured by assessing the variance between
labels of independent labelers, by quality checks on (simulated)
data with known exact labels, or via aleatoric uncertainty. 
In order to assess the \emph{robustness and generalization} ability of the DNNs,
the metrics do not differ significantly and can be summarized as
performance metrics. 
The main difference concerns the input data as described below. 
Common performance metrics
can be found in \cite{cluzeau_concepts_2020}.
The correct choice of performance metrics is highly dependent on the
DNN output and objective \cite{cluzeau_concepts_2020}.
For measurement of generalization ability, the difference between test
and training data distribution is crucial,\eg if only rare poses
are selected, metrics thresholds must be adapted accordingly.
For measurement of robustness it is important to include perturbations
in the input data. These perturbations can be sensor noise such as
dust, dirt, natural domain noise like overexposure,fog etc.
(\cf \cite{michaelis_benchmarking_2020}).
Depending on the extent of such perturbations, a lower performance
threshold is acceptable.
Robustness evaluation techniques in the context of autonomous driving
are reviewed in \cite{michaelis_benchmarking_2020}. 
One of the major disadvantages of DNNs is their black-box
characteristic. All metrics that shed more light on the black box
belong to the metrics of \emph{interpretability}.


